Limiting behaviour of moving average processes genenrated by negatively dependent random variables under sub-linear expectations

Let $\{Y_i,-\infty<i<\infty\}$ be a doubly infinite sequence of identically distributed, negatively dependent random variables under sub-linear expectations, $\{a_i,-\infty<i<\infty\}$ be an absolutely summable sequence of real numbers. In this article, we study complete convergence and Marcinkiewicz-Zygmund strog law of large numbers for the partial sums of moving average processes $\{X_n=\sum_{i=-\infty}^{\infty}a_{i}Y_{i+n},n\ge 1\}$ based on the sequence $\{Y_i,-\infty<i<\infty\}$ of identically distributed, negatively dependent random variables under sub-linear expectations, complementing the result of [Chen, et al., 2009. Limiting behaviour of moving average processes under $\varphi$-mixing assumption. Statist. Probab. Lett. 79, 105-111].

==> elsarticle-harv.bst.tex <==
%%
%% This is file `elsarticle-harv.bst'  (Version 2.1),
%% 
%% Copyright 2009-2020 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%%
%% $Id: elsarticle-harv.bst 194 2020-11-23 11:29:27Z rishi $
%%
%% $URL: https://lenova.river-valley.com/svn/elsarticle/trunk/elsarticle-harv.bst $
%% 

ENTRY
{ address
	archive
	author
	booktitle
	chapter
	collaboration
	edition
	editor
	howpublished
	institution
	journal
	key
	month
	note
	number
	organization
	pages
	publisher
	school
	series
	title
	type
	volume
	year
	url
	doi
	eprint
	pubmed
}
{}
{ label extra.label sort.label short.list }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

STRINGS { urlprefix doiprefix eprintprefix pubmedprefix }

FUNCTION {init.web.variables}
{
	"\URLprefix "     'urlprefix :=
	"\DOIprefix"      'doiprefix :=
	"\ArXivprefix  "   'eprintprefix :=
	"\Pubmedprefix "  'pubmedprefix :=
}

FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
	#2 'after.sentence :=
	#3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.comma}
{ ", " * write$}

FUNCTION {output.nonnull}
{ 's :=
	output.state mid.sentence =
	{ ". " * write$ }
	{ output.state after.block =
		{ add.period$ write$
			newline$
			"\newblock " write$
		}
		{ output.state before.all =
			'write$
			{ ", " * write$ }
			if$
		}
		if$
		mid.sentence 'output.state :=
	}
	if$
	s
}
FUNCTION {output.commanull}
{ 's :=
	output.state mid.sentence =
	{ ", " * write$ }
	{ output.state after.block =
		{ ", " * write$
			newline$
			"\newblock " write$
		}
		{ output.state before.all =
			'write$
			{ add.period$ " " * write$ }
			if$
		}
		if$
		mid.sentence 'output.state :=
	}
	if$
	s
}
FUNCTION {output}
{ duplicate$ empty$
	'pop$
	'output.nonnull
	if$
}
FUNCTION {output.check}
{ 't :=
	duplicate$ empty$
	{ pop$ "empty " t * " in " * cite$ * warning$ }
	'output.nonnull
	if$
}
FUNCTION {output.book.check}
{ 't :=
	duplicate$ empty$
	{ pop$ "empty " t * " in " * cite$ * warning$ }
	'output.nonnull
	if$
}
FUNCTION {fin.entry}
{ add.period$
	write$
	newline$
}

FUNCTION {new.block}
{ output.state before.all =
	'skip$
	{ after.block 'output.state := }
	if$
}
FUNCTION {new.sentence}
{ output.state after.block =
	'skip$
	{ output.state before.all =
		'skip$
		{ after.sentence 'output.state := }
		if$
	}
	if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
	new.block
}

FUNCTION {not}
{   { #0 }
	{ #1 }
	if$
}
FUNCTION {and}
{   'skip$
	{ pop$ #0 }
	if$
}
FUNCTION {or}
{   { pop$ #1 }
	'skip$
	if$
}
FUNCTION {new.block.checkb}
{ empty$
	swap$ empty$
	and
	'skip$
	'new.block
	if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
	{ pop$ "" }
	'skip$
	if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
	{ pop$ "" }
	{ "\textit{" swap$ * "}" * }
	if$
}
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
	{ "~" }
	{ " " }
	if$
	swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
% Here are the language-specific definitions for explicit words.
% Each function has a name bbl.xxx where xxx is the English word.
% The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "Eds." }

FUNCTION {bbl.editor}
{ "Ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "volume" }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "number" }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "pp." }

FUNCTION {bbl.page}
{ "p." }

FUNCTION {bbl.chapter}
{ "chapter" }

FUNCTION {bbl.techrep}
{ "Technical Report" }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"January"}

MACRO {feb} {"February"}

MACRO {mar} {"March"}

MACRO {apr} {"April"}

MACRO {may} {"May"}

MACRO {jun} {"June"}

MACRO {jul} {"July"}

MACRO {aug} {"August"}

MACRO {sep} {"September"}

MACRO {oct} {"October"}

MACRO {nov} {"November"}

MACRO {dec} {"December"}

MACRO {acmcs} {"ACM Comput. Surv."}

MACRO {acta} {"Acta Inf."}

MACRO {cacm} {"Commun. ACM"}

MACRO {ibmjrd} {"IBM J. Res. Dev."}

MACRO {ibmsj} {"IBM Syst.~J."}

MACRO {ieeese} {"IEEE Trans. Software Eng."}

MACRO {ieeetc} {"IEEE Trans. Comput."}

MACRO {ieeetcad}
{"IEEE Trans. Comput. Aid. Des."}

MACRO {ipl} {"Inf. Process. Lett."}

MACRO {jacm} {"J.~ACM"}

MACRO {jcss} {"J.~Comput. Syst. Sci."}

MACRO {scp} {"Sci. Comput. Program."}

MACRO {sicomp} {"SIAM J. Comput."}

MACRO {tocs} {"ACM Trans. Comput. Syst."}

MACRO {tods} {"ACM Trans. Database Syst."}

MACRO {tog} {"ACM Trans. Graphic."}

MACRO {toms} {"ACM Trans. Math. Software"}

MACRO {toois} {"ACM Trans. Office Inf. Syst."}

MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}

MACRO {tcs} {"Theor. Comput. Sci."}

FUNCTION {bibinfo.check}
{ swap$
	duplicate$ missing$
	{
		pop$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ pop$
		}
		{ swap$
			"\bibinfo{" swap$ * "}{" * swap$ * "}" *
		}
		if$
	}
	if$
}
FUNCTION {bibinfo.warn}
{ swap$
	duplicate$ missing$
	{
		swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
		""
	}
	{ duplicate$ empty$
		{
			swap$ "empty " swap$ * " in " * cite$ * warning$
		}
		{ swap$
			pop$
		}
		if$
	}
	if$
}

STRINGS  { bibinfo}

INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
	duplicate$ empty$ 'skip$ {
		's :=
		"" 't :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{vv~}{ll}{, jj}{, f{.}.}"
			format.name$
			bibinfo bibinfo.check
			't :=
			nameptr #1 >
			{
				namesleft #1 >
				{ ", " * t * }
				{
					"," *
					s nameptr "{ll}" format.name$ duplicate$ "others" =
					{ 't := }
					{ pop$ }
					if$
					t "others" =
					{
						" " * bbl.etal *
					}
					{ " " * t * }
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	} if$
}
FUNCTION {format.names.ed}
{
	format.names
}
FUNCTION {format.key}
{ empty$
	{ key field.or.null }
	{ "" }
	if$
}

FUNCTION {format.authors}
{ author "author" format.names
	duplicate$ empty$ 'skip$
	{ collaboration "collaboration" bibinfo.check
		duplicate$ empty$ 'skip$
		{ " (" swap$ * ")" * }
		if$
		*
	}
	if$
}

FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
	{
		" " *
		get.bbl.editor
		capitalize
		"(" swap$ * ")" *
		*
	}
	if$
}
FUNCTION {format.note}
{
	note empty$
	{ "" }
	{ note #1 #1 substring$
		duplicate$ "{" =
			'skip$
			{ output.state mid.sentence =
				{ "l" }
				{ "u" }
				if$
				change.case$
			}
			if$
			note #2 global.max$ substring$ * "note" bibinfo.check
		}
		if$
	}
	
	FUNCTION {format.title}
	{ title
		duplicate$ empty$ 'skip$
		{ "t" change.case$ }
		if$
		"title" bibinfo.check
	}
	FUNCTION {format.full.names}
	{'s :=
		"" 't :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{vv~}{ll}" format.name$
			't :=
			nameptr #1 >
			{
				namesleft #1 >
				{ ", " * t * }
				{
					s nameptr "{ll}" format.name$ duplicate$ "others" =
					{ 't := }
					{ pop$ }
					if$
					t "others" =
					{
						" " * bbl.etal *
					}
					{
						bbl.and
						space.word * t *
					}
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	}
	
	FUNCTION {author.editor.key.full}
	{ author empty$
		{ editor empty$
			{ key empty$
				{ cite$ #1 #3 substring$ }
				'key
				if$
			}
			{ editor format.full.names }
			if$
		}
		{ author format.full.names }
		if$
	}
	
	FUNCTION {author.key.full}
	{ author empty$
		{ key empty$
			{ cite$ #1 #3 substring$ }
			'key
			if$
		}
		{ author format.full.names }
		if$
	}
	
	FUNCTION {editor.key.full}
	{ editor empty$
		{ key empty$
			{ cite$ #1 #3 substring$ }
			'key
			if$
		}
		{ editor format.full.names }
		if$
	}
	
	FUNCTION {make.full.names}
	{ type$ "book" =
		type$ "inbook" =
		or
		'author.editor.key.full
		{ type$ "proceedings" =
			'editor.key.full
			'author.key.full
			if$
		}
		if$
	}
	
	FUNCTION {output.bibitem}
	{ newline$
		"\bibitem[{" write$
			label write$
			")" make.full.names duplicate$ short.list =
			{ pop$ }
			{ * }
			if$
			"}]{" * write$
			cite$ write$
			"}" write$
		newline$
		""
		before.all 'output.state :=
	}
	
	FUNCTION {n.dashify}
	{
		't :=
		""
		{ t empty$ not }
		{ t #1 #1 substring$ "-" =
			{ t #1 #2 substring$ "--" = not
				{ "--" *
					t #2 global.max$ substring$ 't :=
				}
				{   { t #1 #1 substring$ "-" = }
					{ "-" *
						t #2 global.max$ substring$ 't :=
					}
					while$
				}
				if$
			}
			{ t #1 #1 substring$ *
				t #2 global.max$ substring$ 't :=
			}
			if$
		}
		while$
	}
	
	FUNCTION {word.in}
	{ bbl.in %capitalize
		":" *
		" " * }
	
	FUNCTION {format.date}
	{ year "year" bibinfo.check duplicate$ empty$
		{
		}
		'skip$
		if$
		extra.label *
		before.all 'output.state :=
		", " swap$ *
	}
	FUNCTION {format.btitle}
	{ title "title" bibinfo.check
		duplicate$ empty$ 'skip$
		{
		}
		if$
	}
	FUNCTION {either.or.check}
	{ empty$
		'pop$
		{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
		if$
	}
	FUNCTION {format.bvolume}
	{ volume empty$
		{ "" }
		{ bbl.volume volume tie.or.space.prefix
			"volume" bibinfo.check * *
			series "series" bibinfo.check
			duplicate$ empty$ 'pop$
			{ swap$ bbl.of space.word * swap$
				emphasize * }
			if$
			"volume and number" number either.or.check
		}
		if$
	}
	FUNCTION {format.number.series}
	{ volume empty$
		{ number empty$
			{ series field.or.null }
			{ series empty$
				{ number "number" bibinfo.check }
				{ output.state mid.sentence =
					{ bbl.number }
					{ bbl.number capitalize }
					if$
					number tie.or.space.prefix "number" bibinfo.check * *
					bbl.in space.word *
					series "series" bibinfo.check *
				}
				if$
			}
			if$
		}
		{ "" }
		if$
	}
	
	FUNCTION {format.edition}
	{ edition duplicate$ empty$ 'skip$
		{
			output.state mid.sentence =
			{ "l" }
			{ "t" }
			if$ change.case$
			"edition" bibinfo.check
			" " * bbl.edition *
		}
		if$
	}
	INTEGERS { multiresult }
	FUNCTION {multi.page.check}
	{ 't :=
		#0 'multiresult :=
		{ multiresult not
			t empty$ not
			and
		}
		{ t #1 #1 substring$
			duplicate$ "-" =
			swap$ duplicate$ "," =
			swap$ "+" =
			or or
			{ #1 'multiresult := }
			{ t #2 global.max$ substring$ 't := }
			if$
		}
		while$
		multiresult
	}
	%FUNCTION {format.pages}
	%{ pages duplicate$ empty$ 'skip$
		%    { duplicate$ multi.page.check
			%        {
				%          n.dashify
				%        }
			%        {
				%        }
			%      if$
			%      "pages" bibinfo.check
			%    }
		%  if$
		%}
	
	FUNCTION {format.pages}
	{ pages duplicate$ empty$ 'skip$
		{ duplicate$ multi.page.check
			{
				bbl.pages swap$
				n.dashify
			}
			{
				bbl.page swap$
			}
			if$
			tie.or.space.prefix
			"pages" bibinfo.check
			* *
		}
		if$
	}
	
	FUNCTION {format.journal.pages}
	{ pages duplicate$ empty$ 'pop$
		{ swap$ duplicate$ empty$
			{ pop$ pop$ format.pages }
			{
				", " *
				swap$
				n.dashify
				"pages" bibinfo.check
				*
			}
			if$
		}
		if$
	}
	FUNCTION {format.vol.num.pages}
	{ volume field.or.null
		duplicate$ empty$ 'skip$
		{
			"volume" bibinfo.check
		}
		if$
	}
	
	FUNCTION {format.chapter.pages}
	{ chapter empty$
		{ "" }
		{ type empty$
			{ bbl.chapter }
			{ type "l" change.case$
				"type" bibinfo.check
			}
			if$
			chapter tie.or.space.prefix
			"chapter" bibinfo.check
			* *
		}
		if$
	}
	
	FUNCTION {format.booktitle}
	{
		booktitle "booktitle" bibinfo.check
	}
	FUNCTION {format.in.ed.booktitle}
	{ format.booktitle duplicate$ empty$ 'skip$
		{
			editor "editor" format.names.ed duplicate$ empty$ 'pop$
			{
				" " *
				get.bbl.editor
				capitalize
				"(" swap$ * "), " *
				* swap$
				* }
			if$
			word.in swap$ *
		}
		if$
	}
	FUNCTION {format.thesis.type}
	{ type duplicate$ empty$
		'pop$
		{ swap$ pop$
			"t" change.case$ "type" bibinfo.check
		}
		if$
	}
	FUNCTION {format.tr.number}
	{ number "number" bibinfo.check
		type duplicate$ empty$
		{ pop$ bbl.techrep }
		'skip$
		if$
		"type" bibinfo.check
		swap$ duplicate$ empty$
		{ pop$ "t" change.case$ }
		{ tie.or.space.prefix * * }
		if$
	}
	FUNCTION {format.article.crossref}
	{
		word.in
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.book.crossref}
	{ volume duplicate$ empty$
		{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
			pop$ word.in
		}
		{ bbl.volume
			capitalize
			swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
		}
		if$
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.incoll.inproc.crossref}
	{
		word.in
		" \cite{" * crossref * "}" *
	}
	FUNCTION {format.org.or.pub}
	{ 't :=
		""
		address empty$ t empty$ and
		'skip$
		{
			t empty$
			{ address "address" bibinfo.check *
			}
			{ t *
				address empty$
				'skip$
				{ ", " * address "address" bibinfo.check * }
				if$
			}
			if$
		}
		if$
	}
	FUNCTION {format.publisher.address}
	{ publisher "publisher" bibinfo.check format.org.or.pub
	}
	
	FUNCTION {format.organization.address}
	{ organization "organization" bibinfo.check format.org.or.pub
	}
	
	FUNCTION {print.url}
	{url duplicate$ empty$
		{ pop$ "" }
		{ new.sentence
			urlprefix "\url{" * swap$  * "}" *
		}
		if$
	}
	
	FUNCTION {print.doi}
	{doi duplicate$ empty$
		{ pop$ "" }
		{ new.sentence
			doiprefix "\doi{" * swap$  * "}" *
		}
		if$
	}
	
	FUNCTION {print.eprint}
	{eprint duplicate$ empty$
		{ pop$ "" }
		{ new.sentence
			duplicate$ "\href{http://arxiv.org/abs/" swap$ * "}{{\tt arXiv:" * swap$ * "}}" *   }
		if$
	}
	
	FUNCTION {print.pubmed}
	{pubmed duplicate$ empty$
		{ pop$ "" }
		{ new.sentence
			pubmedprefix "\Pubmed{" * swap$  * "}" *
		}
		if$
	}
	
	FUNCTION {webpage}
	{ "%Type = Webpage" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		author empty$
		{
			format.title "title" output.check
			new.block
			format.date "year" output.check
			date.block
		}
		{
			format.date "year" output.check
			date.block
			format.title "title" output.check
			new.block
		}
		if$
		print.url output
		fin.entry
	}
	
	
	FUNCTION {article}
	{ "%Type = Article" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.title "title" output.check
		new.block
		crossref missing$
		{
			journal
			"journal" bibinfo.check
			"journal" output.check
			add.blank
			format.vol.num.pages output
		}
		{ format.article.crossref output.nonnull
		}
		if$
		format.journal.pages
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {book}
	{ "%Type = Book" write$
		output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
			editor format.key output
		}
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		crossref missing$
		{ format.bvolume output
			new.block
			format.number.series output
			format.edition output
			new.sentence
			format.publisher.address output
		}
		{
			new.block
			format.book.crossref output.nonnull
		}
		if$
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {booklet}
	{ "%Type = Booklet" write$
		output.bibitem
		format.authors output
		author format.key output
		format.date "year" output.check
		date.block
		format.title "title" output.check
		new.block
		howpublished "howpublished" bibinfo.check output
		address "address" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {inbook}
	{ "%Type = Inbook" write$
		output.bibitem
		author empty$
		{ format.editors "author and editor" output.check
			editor format.key output
		}
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		format.edition output
		crossref missing$
		{
			format.publisher.address output
			format.bvolume output
			format.chapter.pages "chapter and pages" output.check
			new.block
			format.number.series output
			new.sentence
		}
		{
			format.chapter.pages "chapter and pages" output.check
			new.block
			format.book.crossref output.nonnull
		}
		if$
		format.pages "pages" output.check
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {incollection}
	{ "%Type = Incollection" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.title "title" output.book.check
		new.sentence
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.book.check
			format.edition output
			format.publisher.address output
			format.bvolume output
			format.number.series output
			format.chapter.pages output
			new.sentence
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.chapter.pages output
		}
		if$
		format.pages "pages" output.check
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {inproceedings}
	{ "%Type = Inproceedings" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.title "title" output.book.check
		new.sentence
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.check
			new.sentence
			publisher empty$
			{ format.organization.address output }
			{ organization "organization" bibinfo.check output
				format.publisher.address output
			}
			if$
			%      format.bvolume output
			%      format.number.series output
			%      format.pages output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.pages output
		}
		if$
		format.pages "pages" output.check
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {conference} { inproceedings }
	
	FUNCTION {manual}
	{ "%Type = Manual" write$
		output.bibitem
		format.authors output
		author format.key output
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		format.edition output
		organization address new.block.checkb
		organization "organization" bibinfo.check output
		address "address" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {mastersthesis}
	{ "%Type = Masterthesis" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.btitle
		"title" output.check
		new.block
		bbl.mthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {misc}
	{ "%Type = Misc" write$
		output.bibitem
		format.authors output
		author format.key output
		format.date "year" output.check
		date.block
		format.title output
		new.block
		howpublished "howpublished" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {phdthesis}
	{ "%Type = Phdthesis" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.btitle
		"title" output.check
		new.block
		bbl.phdthesis format.thesis.type output.nonnull
		school "school" bibinfo.warn output
		address "address" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {proceedings}
	{ "%Type = Proceedings" write$
		output.bibitem
		format.editors output
		editor format.key output
		format.date "year" output.check
		date.block
		format.btitle "title" output.check
		format.bvolume output
		format.number.series output
		new.sentence
		publisher empty$
		{ format.organization.address output }
		{ organization "organization" bibinfo.check output
			format.publisher.address output
		}
		if$
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {techreport}
	{ "%Type = Techreport" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.btitle
		"title" output.check
		new.block
		format.tr.number output.nonnull
		institution "institution" bibinfo.warn output
		address "address" bibinfo.check output
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note output
		fin.entry
	}
	
	FUNCTION {unpublished}
	{ "%Type = Unpublished" write$
		output.bibitem
		format.authors "author" output.check
		author format.key output
		format.date "year" output.check
		date.block
		format.title "title" output.check
		new.block
		print.url output
		print.doi output
		print.eprint output
		print.pubmed output
		format.note "note" output.check
		fin.entry
	}
	
	FUNCTION {default.type} { misc }
	READ
	FUNCTION {sortify}
	{ purify$
		"l" change.case$
	}
	INTEGERS { len }
	FUNCTION {chop.word}
	{ 's :=
		'len :=
		s #1 len substring$ =
		{ s len #1 + global.max$ substring$ }
		's
		if$
	}
	FUNCTION {format.lab.names}
	{ 's :=
		"" 't :=
		s #1 "{vv~}{ll}" format.name$
		s num.names$ duplicate$
		#2 >
		{ pop$
			" " * bbl.etal *
		}
		{ #2 <
			'skip$
			{ s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
				{
					" " * bbl.etal *
				}
				{ bbl.and space.word * s #2 "{vv~}{ll}" format.name$
					* }
				if$
			}
			if$
		}
		if$
	}
	
	FUNCTION {author.key.label}
	{ author empty$
		{ key empty$
			{ cite$ #1 #3 substring$ }
			'key
			if$
		}
		{ author format.lab.names }
		if$
	}
	
	FUNCTION {author.editor.key.label}
	{ author empty$
		{ editor empty$
			{ key empty$
				{ cite$ #1 #3 substring$ }
				'key
				if$
			}
			{ editor format.lab.names }
			if$
		}
		{ author format.lab.names }
		if$
	}
	
	FUNCTION {editor.key.label}
	{ editor empty$
		{ key empty$
			{ cite$ #1 #3 substring$ }
			'key
			if$
		}
		{ editor format.lab.names }
		if$
	}
	
	FUNCTION {calc.short.authors}
	{ type$ "book" =
		type$ "inbook" =
		or
		'author.editor.key.label
		{ type$ "proceedings" =
			'editor.key.label
			'author.key.label
			if$
		}
		if$
		'short.list :=
	}
	
	FUNCTION {calc.label}
	{ calc.short.authors
		short.list
		"("
		*
		year duplicate$ empty$
		short.list key field.or.null = or
		{ pop$ "" }
		'skip$
		if$
		*
		'label :=
	}
	
	FUNCTION {sort.format.names}
	{ 's :=
		#1 'nameptr :=
		""
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr
			"{ll{ }}{  f{ }}{  jj{ }}"
			format.name$ 't :=
			nameptr #1 >
			{
				"   "  *
				namesleft #1 = t "others" = and
				{ "zzzzz" * }
				{ t sortify * }
				if$
			}
			{ t sortify * }
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	}
	
	FUNCTION {sort.format.title}
	{ 't :=
		"A " #2
		"An " #3
		"The " #4 t chop.word
		chop.word
		chop.word
		sortify
		#1 global.max$ substring$
	}
	FUNCTION {author.sort}
	{ author empty$
		{ key empty$
			{ "to sort, need author or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ author sort.format.names }
		if$
	}
	FUNCTION {author.editor.sort}
	{ author empty$
		{ editor empty$
			{ key empty$
				{ "to sort, need author, editor, or key in " cite$ * warning$
					""
				}
				{ key sortify }
				if$
			}
			{ editor sort.format.names }
			if$
		}
		{ author sort.format.names }
		if$
	}
	FUNCTION {editor.sort}
	{ editor empty$
		{ key empty$
			{ "to sort, need editor or key in " cite$ * warning$
				""
			}
			{ key sortify }
			if$
		}
		{ editor sort.format.names }
		if$
	}
	FUNCTION {presort}
	{ calc.label
		label sortify
		"    "
		*
		type$ "book" =
		type$ "inbook" =
		or
		'author.editor.sort
		{ type$ "proceedings" =
			'editor.sort
			'author.sort
			if$
		}
		if$
		#1 entry.max$ substring$
		'sort.label :=
		sort.label
		*
		"    "
		*
		title field.or.null
		sort.format.title
		*
		#1 entry.max$ substring$
		'sort.key$ :=
	}
	
	ITERATE {presort}
	SORT
	STRINGS { last.label next.extra }
	INTEGERS { last.extra.num number.label }
	FUNCTION {initialize.extra.label.stuff}
	{ #0 int.to.chr$ 'last.label :=
		"" 'next.extra :=
		#0 'last.extra.num :=
		#0 'number.label :=
	}
	FUNCTION {forward.pass}
	{ last.label label =
		{ last.extra.num #1 + 'last.extra.num :=
			last.extra.num int.to.chr$ 'extra.label :=
		}
		{ "a" chr.to.int$ 'last.extra.num :=
			"" 'extra.label :=
			label 'last.label :=
		}
		if$
		number.label #1 + 'number.label :=
	}
	FUNCTION {reverse.pass}
	{ next.extra "b" =
		{ "a" 'extra.label := }
		'skip$
		if$
		extra.label 'next.extra :=
		extra.label
		duplicate$ empty$
		'skip$
		%    { "{\natexlab{" swap$ * "}}" * }
		{ "" swap$ * "" * }
		if$
		'extra.label :=
		label extra.label * 'label :=
	}
	EXECUTE {initialize.extra.label.stuff}
	ITERATE {forward.pass}
	REVERSE {reverse.pass}
	FUNCTION {bib.sort.order}
	{ sort.label
		"    "
		*
		year field.or.null sortify
		*
		"    "
		*
		title field.or.null
		sort.format.title
		*
		#1 entry.max$ substring$
		'sort.key$ :=
	}
	ITERATE {bib.sort.order}
	SORT
	FUNCTION {begin.bib}
	{ preamble$ empty$
		'skip$
		{ preamble$ write$ newline$ }
		if$
		"\begin{thebibliography}{" number.label int.to.str$ * "}" *
			write$ newline$
			"\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi"
			write$ newline$
			"\providecommand{\url}[1]{\texttt{#1}}"
			write$ newline$
			"\providecommand{\href}[2]{#2}"
			write$ newline$
			"\providecommand{\path}[1]{#1}"
			write$ newline$
			"\providecommand{\DOIprefix}{doi:}"
			write$ newline$
			"\providecommand{\ArXivprefix}{arXiv:}"
			write$ newline$
			"\providecommand{\URLprefix}{URL: }"
			write$ newline$
			"\providecommand{\Pubmedprefix}{pmid:}"
			write$ newline$
			"\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}"
			write$ newline$
			"\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}"
			write$ newline$
			"\providecommand{\bibinfo}[2]{#2}"
			write$ newline$
			"\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi"
			write$ newline$
		}
		EXECUTE {begin.bib}
		EXECUTE {init.state.consts}
		EXECUTE {init.web.variables} 
		ITERATE {call.type$}
		FUNCTION {end.bib}
		{ newline$
			"\end{thebibliography}" write$ newline$
	}
	EXECUTE {end.bib}
	%% End of customized bst file
	%%
	%% End of file `elsarticle-harv.bst'.
	%%
	%% Change log:
	%% -----------
	%% 22.04.2011
	%%
	%% 10.08.2012
	%%   a. doi, url, eprint, pmid added
	%%   b. Bibtype `webpage' defined
	%%
	%% 30.08.2012
	%%   a. collaboration added.
	%%
	

